Towards Learning of Filter-Level Heterogeneous Compression of Convolutional Neural Networks

Recently, deep learning has become a de facto standard in machine learning with convolutional neural networks (CNNs) demonstrating spectacular success on a wide variety of tasks. However, CNNs are typically very demanding computationally at inference time. One of the ways to alleviate this burden on certain hardware platforms is quantization relying on the use of low-precision arithmetic representation for the weights and the activations. Another popular method is the pruning of the number of filters in each layer. While mainstream deep learning methods train the neural networks weights while keeping the network architecture fixed, the emerging neural architecture search (NAS) techniques make the latter also amenable to training. In this paper, we formulate optimal arithmetic bit length allocation and neural network pruning as a NAS problem, searching for the configurations satisfying a computational complexity budget while maximizing the accuracy. We use a differentiable search method based on the continuous relaxation of the search space proposed by Liu et al. (arXiv:1806.09055). We show, by grid search, that heterogeneous quantized networks suffer from a high variance which renders the benefit of the search questionable. For pruning, improvement over homogeneous cases is possible, but it is still challenging to find those configurations with the proposed method. The code is publicly available at https://github.com/yochaiz/Slimmable and https://github.com/yochaiz/darts-UNIQ

==> definitions.tex <==
\section{Definitions}

$\layerOpsSet$ - represents layer $\ell$ operations set, \ie $\layerOpsSet = \{ (2,2), (3,3) \}$ \\
$\nConfig$ - number of configurations for layer $\ell$. \\
$\nFiltersLayer$ - total number of filters in layer $\ell$. \\
$\configSubset{k}$ - configurations subset in iteration $k$ for gradient estimation. \\
$\networkConfig$ - denotes a network configuration. \\
$\networkComplexity$ - denotes network configuration arithmetic complexity. \\
$\homogeneousConfig{t}$ - denotes homogeneous configurations. \\
$\homogeneousComplexity{t}$ - denotes homogeneous configurations arithmetic complexity. \\
$\networkWeights$ - denotes network weights set. \\
$\configWeights$ - denotes a specific weights set for a specific configuration $\networkConfig$. \\
$\trainSet$ - denotes the whole training data set. \\
$\searchSet$ - denotes search data set, data set for $\prob$ optimization. \\
$\trainWeightsSet$ - denotes data set for weights training. \\
$\trainWeightsEpochs$ - denotes number of epochs for weights training. \\
$\trainWeightsInterval$ - denotes once in how many iterations to train weights. \\
$\probConfig$ - denotes the probability to sample configuration $\networkConfig$ from distribution $\prob$. \\
$\Loss$ - denotes the loss function, \ie target function we want to optimize. \\
$\prob$ - denotes a distribution. \\
$\lossConfig$ - denotes the loss for configuration $\networkConfig$. \\
$\expectedValue{k}$ - denotes the expected value of distrubtion $\prob$ at iteration $k$. \\
$\expectedConfig{}$ - denotes the configuration of the $\prob$ distribution expected value. \\
$\lossExpectedValue$ - loss expected value under distribution $\prob$. \\
$\ceLoss$ - cross entropy loss for configuration $\networkConfig$. \\
$\ceLossInterpolation{\networkConfig}$ - the expected cross entropy loss for configuration $\networkConfig$ as the interpolation between the cross entropy loss of configurations $h_1,h_2$. \\
$\complexitySigma$ - the function we apply on $\networkComplexity$. \\
$\complexityLoss$ - arithmetic complexity loss for configuration $\networkConfig$. \\
$\configsSum$ - the target function expected value as sum of losses multiplied by their probabilities. \\
$\opAlpha{i}$ - $\alpha$ value for operation $i$ in layer $\ell$. A notation for the multinomial case. \\
$\opAlphaSingle$ - $\alpha$ value for operation (random variable) $i$ in layer $\ell$. A notation for the binomial case, \ie a single random variable in each layer. \\
$\opSample{i}$ - the number of filters in layer $\ell$ we apply operation $i$ on. A notation for the multinomial case. \\
$\opSampleSingle$ - the number of filters we select in layer $\ell$. A notation for the binomial case. \\
$\opProb{i}$ - the probability to select operation $i$ in layer $\ell$. A notation for the multinomial case. \\
$\opProbSingle$ - The probability of layer $\ell$ random variable. A notation for the binomial case. \\
$\opDerivative{i}$ - $\J$ derivative with respect to $\opAlpha{i}$. A notation for the multinomial case. \\
$\opDerivativeSingle$ - $\J$ derivative with respect to $\opAlphaSingle$. A notation for the binomial case. \\
$\opDerivativeEstimator{i}$ - $\opDerivative{i}$ estimator. \\
$\opProbDetailed{i}$ - detailed probability term for operation $i$ in layer $\ell$. A notation for the multinomial case. \\
$\layerConfig{k}$ - a specific layer configuration. \\
$\layerRV{\ell}$ - random variable (multinomial or binomial) for layer $\ell$. \\
$\layerConfigDetailed$ - detailed version of layer $\ell$ configuration, \ie number of filters assigned for each operation. A notation for the multinomial case. \\
$\layerConfigSingleDetailed$ - detailed version of layer $\ell$ configuration, \ie number of filters selected. A notation for the binomial case. \\
$\bitWeights$ - number of bits used for filter weights quantization. \\
$\bitActivations$ - number of bits used for layer output (activation) quantization. \\
$\layerConfigProb$ - The probability to sample configuration $\layerConfig{\ell}$ in layer $\ell$. 
\begin{itemize}
    \item $\multinomialConfigProb$ - explicit term for $\layerConfigProb$ in the multinomial case.
    \item $\multinomialFrac$
    \item $\multinomialConfigProbFrac$
    \item $\opSampleNumeratorMultinomial$
    \item $\opSampleNumeratorMultinomialSum$
    \item $\opSampleDenominatorMultinomial$
    \item $\opSampleDenominatorMultinomialWithPower$
\end{itemize}
$\opAlphaDerivative$ - derivation with respect to $\opAlpha{t}$. A notation for the multinomial case. \\
$\opAlphaSingleDerivative$ - derivation with respect to $\opAlphaSingle$. A notation for the binomial case. \\
$\multinomialConfigDerivative$ - layer $\ell$ configuration derivative with respect to $\opAlpha{t}$. \\
$\prodLayersProbLeaveOut{k}$ - The probability to choose configuration in any layer except layer $\ell$. \\
$\multinomialConfigProbDerivative{k}$ - configuration $\networkConfig$ derivative with respect to $\opAlpha{t}$. \\
$\multinomialLossEVderivative$ - $\J$ derivative with respect to $\opAlpha{t}$. \\
$\nTrialsBinomial$ - number of trials for a Binomial random variable. \\
\begin{itemize}
    \item $\binomialConfigProb$ - explicit term for $\layerConfigProb$ in the binomial case.
    \item $\binomialFrac$
    \item $\binomialConfigProbFrac$
    \item $\opProbBinomialDetailedNumeratorWithPower$
    \item $\opProbBinomialDetailedDenominatorWithPower$
    \item $\opProbBinomialDetailedNumerator$
    \item $\opProbBinomialDetailedDenominator$
    \item $\opProbBinomialDetailed$
    \item $\opProbBinomialDetailedWithPower$
    \item $\binomialComplementPower$
\end{itemize}
$\opSampleSingleConfig{}$ - number of filters sampled in layer $\ell$. \\
$\binomialConfigDerivative$ - layer $\ell$ configuration derivative with respect to $\opAlphaSingle$. \\
$\binomialConfigProbDerivative{}$ - configuration $\networkConfig$ derivative with respect to $\opAlphaSingle$. \\
$\binomialLossEVderivative$ - $\J$ derivative with respect to $\opAlphaSingle$. \\

% \def\tdu#1#2#3{#1{}_{{#2}}{}^{{#3}}}
% %%%% MATH %%%%
% \def\oper{{t}}
% \def\loss#1{{\mathcal{L}_{{#1}}}}
% \def\Loss{{\mathcal{L}}}
% \def\ourAlpha{{\theta}}
% \def\bops{{\mathcal{B}}}
% \def\normedAlpha{{\hat{\theta}}} % TODO: Hat?
% \def\vourAlpha{{\bm{\theta}}}
% \def\vnormedAlpha{{\hat{\vourAlpha}}}
% \def\idx{{a}}
% \def\vidx{{\bm{\idx}}} % todo: \ri or \vi
% \def\weights{\bm{\omega}}
% \def\policy{\pi\left(\vidx;\vourAlpha\right)}
% \def\weightLoss{\loss{weights}}
% \def\valLoss{\loss{search}\left(\vidx;\weights\right)}
% \def\totalLoss{\Loss\left(\vidx;\weights\right)}
% \def\bopsLoss{\loss{\bops}\left(\vidx\right)}
% \def\return{J\left(\vourAlpha;\weights\right)}
% \def\Return{J}
% \def\sample#1{{\mathcal{S}_{#1}}}
% \def\operations{T}
% \def\opNum{\abs{\operations}}


% % =====================
% \newcommand{\multinomial}{\text{Multinomial}}
% \newcommand{\binomial}{\text{Binomial}}
% \newcommand{\round}{\text{round}}
